Learning Fast and Slow: PROPEDEUTICA for Real-time Malware Detection

Existing malware detectors on safety-critical devices have difficulties in runtime detection due to the performance overhead. In this paper, we introduce PROPEDEUTICA, a framework for efficient and effective real-time malware detection, leveraging the best of conventional machine learning (ML) and deep learning (DL) techniques. In PROPEDEUTICA, all software start execution are considered as benign and monitored by a conventional ML classifier for fast detection. If the software receives a borderline classification from the ML detector (e.g. the software is 50% likely to be benign and 50% likely to be malicious), the software will be transferred to a more accurate, yet performance demanding DL detector. To address spatial-temporal dynamics and software execution heterogeneity, we introduce a novel DL architecture (DEEPMALWARE) for PROPEDEUTICA with multi-stream inputs. We evaluated PROPEDEUTICA with 9,115 malware samples and 1,338 benign software from various categories for the Windows OS. With a borderline interval of [30%-70%], PROPEDEUTICA achieves an accuracy of 94.34% and a false-positive rate of 8.75%, with 41.45% of the samples moved for DEEPMALWARE analysis. Even using only CPU, PROPEDEUTICA can detect malware within less than 0.1 seconds.

==> bio.tex <==
\vskip -2.5\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/ruimin.png}}]{Ruimin Sun}
is a Postdoctoral Research Associate at Northeastern University. She received her Ph.D. from  the University of Florida. She works on secure, reliable systems, and machine learning model protection. 
\end{IEEEbiography}

% \vskip -2.5\baselineskip plus -1fil
\vspace{-2em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/Xiaoyong-Yuan_rsz.png}}]{Xiaoyong Yuan} is an Assistant Professor at the College of Computing, Michigan Technological University. He received the B.S. degree from Fudan University, in 2012, the M.E. degree from Peking University, in 2015, and the Ph.D. degree from the University of Florida, in 2020. His research interests lie in deep learning, security \& privacy, and cloud computing.
\end{IEEEbiography}
\vspace{-2em}
% \vskip -2.5\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/pan.png}}]{Pan He} received his B.E. in Software Engineering from Sichuan University in 2015. He is pursuing a Ph.D. degree in Computer Science at the University of Florida. His current research is focused on understanding the three-dimensional motion and structure of a dynamic scene via developing deep learning methods in various environments.
\end{IEEEbiography}

% \vskip -2.5\baselineskip plus -1fil
\vspace{-2em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/qile.jpg}}]{Qile Zhu}
received Ph.D. from the Department of Computer \& Information Science \& Engineering at the University of Florida in 2020. His research interests include deep learning and natural language processing. He received a B.E. degree from Zhejiang University in 2013 and a master degree from the University of Florida in 2015.
\end{IEEEbiography}

\vspace{-2em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/aokun.jpeg}}]{Aokun Chen} is a Postdoctoral Researcher under the supervise of Dr. Guo at the University of Florida (UF). He received his Ph.D. degree in Computer Engineering on machine learning for security systems from UF. His current research interests include machine learning for bioinformatics and cybersecurity.
\end{IEEEbiography}

% \vskip -2.5\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/andre.png}}]{Andr\'e Gr\'egio} is an Assistant Professor at the Federal University of Paran\'a (UFPR). His research intersects computer security and data science, e.g., effective malware analysis and attack detection systems.
% He is a member of the Network, Distributed Systems, and Security Lab and the Center of Scientific Computing and Free Software at UFPR. His research interests are in systems security and machine learning application to security data. as well as creating machine learning models for clustering and classification of massive, ever-changing security data.
\end{IEEEbiography}
% \vskip -2.5\baselineskip plus -1fil

\vspace{-2em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/daniela.png}}]{Daniela Oliveira} is an Associate Professor at University of Florida (UF). 
% She received her BS and MS degree in Computer Science from the Federal University of Minas Gerais in Brazil. 
% She received her PhD in Computer Science from the University of California at Davis, where she specialized in security and operating systems. 
Her research includes human factors security and IoT security, especially the application of dynamic information flow to thwart attacks.
\end{IEEEbiography}
\vspace{-2em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/andyli.png}}]{Xiaolin (Andy) Li} is Partner of Tongdun Technology, heading the AI Institute; Chair Professor and Chief Scientist of IBMC, Chinese Academy of Sciences. He was a Professor at the University of Florida and founding center director of NSF Center for Big Learning. His research interests include deep learning, cloud computing, security \& privacy, IoT, and intelligent medicine.
\end{IEEEbiography}


==> response.tex <==
\large
\onecolumn
\setcounter{page}{1}
\begin{center}
{\Large\bf Response to Reviewer Comments}
\end{center}

\noindent
Dear Editors and Reviewers, 

\vspace{1em}
Please find enclosed the revision of the paper ``Learning Fast and Slow: \spectrum for Real-time Malware Detection.''
We thank you for providing helpful and constructive comments. All of the comments raised by the reviewers have been addressed and the paper has been revised accordingly.

\vspace{1em}
To facilitate the review process, we highlight the major parts that have been added or modified in the manuscript. A detailed list of revisions is given below.

\vspace{1em}
Thank you for your time and consideration.
% \vspace{1em}
% Yours sincerely, \\
% \vspace{1em}
% Ruimin Sun, Xiaoyong Yuan, Pan He, Qile Zhu, Aokun Chen, Andre Gregio, Daniela Oliveira, Xiaolin Li



\vspace{3em}
\begin{center}
{\Large\bf Response to the Associate Editor}
\end{center}
We would like to thank the editor for taking the time to read and evaluate our work. We have addressed all comments and suggestions provided by the reviewers, which have significantly improved the presentation of our paper. 



\vspace{3em}
\begin{center}
{\Large\bf Response to Reviewer 1}
\end{center}

We would like to thank the reviewer for taking the time to read and evaluate our work. We have addressed all comments and suggestions. 

\vspace{1em}
\noindent
\textbf{Comment 1:} Following up the previous concern 7, the reviewer agrees with what the author stated. However, for table 3, the performance of 2nd row (KDD'17 [22]) only have one metric in term of accuracy, while the others have 3 metrics for performance evolution. It's a little strange. Also, regarding the new added statements for table 3, are the 4 datasets with the same difficulty?

\vspace{1em}
\noindent
\textbf{Response:} The performance in terms of precision and recall is not provided in~\cite{wang2017adversary}. Therefore, we did not include it in Table 3. We added an explanation on this in the paper. 

The features used in our work and the LNCS dataset are Windows system calls. The features used in DMIN and KDD datasets are Windows API calls. System calls used in our paper can provide more insights at the kernel level, compared with Windows API calls at the user level. In addition, our collected dataset consists of much more data samples (traces) than the other three datasets, which provides more accurate evaluation results and detection time guarantee. More importantly, these works only consider offline analysis and lacks analysis of the detection time in real-time. We have revised the comparison and added the detailed description of the datasets in Section~\ref{sec:dl_compare}, which is quoted below for the ease of review.



\vspace{1em}
% \yj{the following is repeated.}
\xyn{The features used in our work and~\cite{kolosnjaji2016deep} are Windows system calls. The features used in~\cite{hardy2016dl4md} and~\cite{wang2017adversary} are Windows API calls. Compared with Window API calls, system calls provide more insight about the software at kernel level, compared with Window API calls collected data in the user level only. Moreover, we evaluate the detection performance on a much larger dataset with more traces evaluated, which provides more accurate evaluation results.}

\vspace{1em}
\noindent
\textbf{Comment 2:} Regarding to the previous concern 2, some additional explanations are needed in the revised manuscript. Previous concern 2: For the proposed model, why it could achieve a real-time detection for malware. The key insight is not clearly stated either in the introduction part or in the methodology part.

\vspace{1em}
\noindent
\textbf{Response:} We have added the explanations in the Introduction and the Methodology sections, which are quoted below for the ease of review.

\vspace{1em}
\xyn{
DL requires more time to gain enough information for classification and to predict the probability of detection.
Moreover, the state-of-the-art DL models consist of deep layers and a huge amount of parameters, which results in slow calculation in the prediction. Such slow process makes DL models infeasible to provide predictions on malware in real time. 
}

\xyn{The main goal of this paper using \spectrum is to present the concept of a multi-stage malware detector that combines two distinct classification
models---ML and DL. By leveraging the fast speed in ML methods and high accuracy in DL methods, \spectrum aims to achieve precise and real-time detection.}

\vspace{1em}
\noindent
\textbf{Comment 3:} For the new added subsession, i.e., V. Discussion - C. Weakly Supervised Anomaly Detection, the authors could also consider to include some latest work of weakly supervised anomaly detection, such as "Feature Encoding with AutoEncoders for Weakly-supervised Anomaly Detection, IEEE Transactions on Neural Networks and Learning Systems, 2021".

\vspace{1em}
\noindent
\textbf{Response:} We have included the latest work of weakly supervised anomaly detection, ``Feature Encoding with AutoEncoders for Weakly-supervised Anomaly Detection,'' (\cite{zhou2021feature}) in the Discussion section. 


\vspace{3em}
\begin{center}
{\Large\bf Response to Reviewer 2}
\end{center}
\textbf{Comment 1:}  I thank the authors for addressing the questions from the previous draft. I recommend the paper for publication.
% \noindent
% We would like to thank the Reviewer for taking the time to read and evaluate our work. We have addressed all comments and suggestions, which have significantly improved the presentation of our paper. \yj{this part might go to the previous paragraph.}

\vspace{1em}
\noindent
\textbf{Response:} We thank the Reviewer for reviewing and positively evaluating our manuscript.


\vspace{3em}
\begin{center}
{\Large\bf Response to Reviewer 3}
\end{center}
We would like to thank the reviewer for taking the time to read and evaluate our work. We have addressed all comments and suggestions. 

\vspace{1em}
\noindent
\textbf{Comment 1:} When first introducing the adversarial machine learning in section 2 on page 2, it is better to give a survey (e.g., Adversarial Examples: Opportunities and Challenges, IEEE Transactions on Neural Networks and Learning Systems, 2020) for reference instead of the technical papers.

\vspace{1em}
\noindent
\textbf{Response:} We replaced the technical papers with the adversarial example survey, ``Adversarial Examples: Opportunities and Challenges'' (\cite{zhang2019adversarial}), in Section 2 to improve the presentation of the paper, which is quoted below for the ease of review.


% \vspace{1em}
% \yj{the following is redundant?}
\xyn{Therefore, attacks either targeting \spectrum's
software implementation, or to the machine
learning engine (adversarial machine
learning~\cite{yuan2019adversarial,zhang2019adversarial}) are outside \spectrum's scope. We discuss the adversarial attacks against malware detection in Section~\ref{sec:adversarial}.}

